Distributed Non-Stochastic Experts

We consider the online distributed non-stochastic experts problem, where the distributed system consists of one coordinator node that is connected to $k$ sites, and the sites are required to communicate with each other via the coordinator. At each time-step $t$, one of the $k$ site nodes has to pick an expert from the set ${1, ..., n}$, and the same site receives information about payoffs of all experts for that round. The goal of the distributed system is to minimize regret at time horizon $T$, while simultaneously keeping communication to a minimum. The two extreme solutions to this problem are: (i) Full communication: This essentially simulates the non-distributed setting to obtain the optimal $O(\sqrt{\log(n)T})$ regret bound at the cost of $T$ communication. (ii) No communication: Each site runs an independent copy : the regret is $O(\sqrt{log(n)kT})$ and the communication is 0. This paper shows the difficulty of simultaneously achieving regret asymptotically better than $\sqrt{kT}$ and communication better than $T$. We give a novel algorithm that for an oblivious adversary achieves a non-trivial trade-off: regret $O(\sqrt{k^{5(1+\epsilon)/6} T})$ and communication $O(T/k^{\epsilon})$, for any value of $\epsilon \in (0, 1/5)$. We also consider a variant of the model, where the coordinator picks the expert. In this model, we show that the label-efficient forecaster of Cesa-Bianchi et al. (2005) already gives us strategy that is near optimal in regret vs communication trade-off.

==> alg_sp.tex <==
\subsection{Non-trivial Algorithm} 
\zl{start of the edit. The parameters $\epsilon_i$ below is at this moment inconsistent 
with the parameters for the theorem. }

\zl{This algorithm works for two experts. We will use a new subsection to generalize the algorithm to $n$ experts.}

Our algorithm works as follows. First, our algorithm divides the input
into blocks so that each block approximately contains $k^{1+\epsilon_1}$ input,
where $\epsilon_1$ is a constant to be decided later. At the beginning of each block,
every site sends the accumulated payoff for both arms to the coordinator
and decide the algorithmic strategy for that block.

Before we move forward to describing the algorithmic strategy,
let us briefly discuss how the distributed system may decide the boundaries
of the blocks. We maintain an approximate $\hyz(\epsilon_0, \delta)$ distributed counter over the coordinator, where
$\epsilon_0 = 0.1$ and $\delta$ is a variable to be decided later.
When the counter reaches $k^{1+\epsilon_1}$, the coordinator will send a message to each of the
sites and let them know the block is completed. The $\hyz(\epsilon_0)$ counter will also reset to $0$
after a block is completed.
Notice that the $\hyz$ counter guarantees that the actual count at the end of each block is between
$(1-\epsilon_0)k^{1+\epsilon_1}$ and $(1+\epsilon_0)k^{1+\epsilon_1}$. In what follows, we shall silently assume the $\hyz$ counter never fails. This can be achieved by setting $\delta$ in $\hyz$ counter sufficiently small so that the fail events will have negligible impact over our distributed algorithm.

Next, let us introduce more notations. We let $b$ be the total number of blocks we see. Let $\vecp^j_i$ be
the payoff vector for the $j$-th input of the $i$-th block. Abusing the notation, we shall sometimes also refer to $\vecp^j_i$
as the input itself. Let $a^j_i$ be the corresponding action for the same input. Let $\ell_i$
be the length of the $i$-th input. We denote the total payoff for the $i$-th block be $\vecP^i$. Also,
the cumulative payoff up to the $i$-th block is denoted as $\vecQ^i$, i.e.
$$\vecP^i = \sum_{j \leq \ell_i}\vecp^j_i \quad \mbox{ and } \quad \vecQ^i = \sum_{j \leq i}\vecP^j.$$

When $\delta$ is sufficiently small, by using $\hyz(\epsilon_0, \delta)$ counter we can guarantee that
with high probability $\ell_i = \Theta(k^{1+\epsilon_1}$ for all $i \leq b$ and $b = \Theta\left(\frac{T}{k^{1+\epsilon_1}}\right)$.

Now we are ready to describe our algorithmic strategy for each of the blocks. Let $q = k^{1+\epsilon_1}\sqrt{\frac{k^{-\epsilon_2}}{T}}$, where $\epsilon_2$ is a parameter to be decided later. Our algorithm runs $\proc{Algo-1}$ for the new block with probability $q$ and runs $\proc{Algo-2}$ with probability $1-q$.

\begin{codebox}
\Procname{$\proc{Algo-1}(\mbox{$i$-th block})$}
\li \For $j \gets 1$ \To $\ell_i$
\li \Do
\li The site receiving the input $\vecp^j_i$ report to the coordinator.
\li Let $\sigma_0, \sigma_1 \leftarrow_{U}[0, \sqrt{k^{1+\epsilon_1}}]$.
\li \If $\sum_{j' < j}\vecp^{j'}_i[0] +\sigma_0 \geq \sum_{j' < j}\vecp^{j'}_i[1]+\sigma_1$
\li \Then the coordinator instruct the site to choose action $0$.
\li \Else the coordinator instruct the site to choose action $1$.
\End
\End
\end{codebox}

\begin{codebox}
\Procname{$\proc{Algo-2}(\mbox{$i$-th block})$}
\li Let $i_1, ..., i_m$ be the blocks that used $\proc{Algo-2}$ before $i$-th block
\li Let $\sigma_0, \sigma_1 \leftarrow_{U}[0, \sqrt{k^{1+\epsilon_1-\epsilon_3}T}]$.
\li \If $\sum_{j < m}\vecP^{i_j}[0] +\sigma_0 \geq \sum_{j < m}\vecP^{i_j}[1]+\sigma_1$
\li \Then the coordinator instruct the sites to always choose action $0$ in this block.
\li \Else the coordinator instruct the sites to always choose action $1$ in this block.
\End
\end{codebox}

Both $\proc{Algo-1}$ and $\proc{Algo-2}$ are variations of the \emph{follow the perturbed leader algorithm} (hereafter, FLP). $\proc{Algo-1}$ runs a new instance of FPL for each of the selected blocks. $\proc{Algo-2}$, on the other hand, treats each big block as a single input and runs the FPL at block level. Notice that the noise we use in $\proc{Algo-2}$ is a non-standard noise: recall that when we use a FPL algorithm for an input sequence of length $\Theta(T/k^{1+\epsilon_1})$, each of which has reward $[0, k^{1+\epsilon_1}]$, then we need to add noises that are uniformly from $[0, \sqrt{k^{1+\epsilon_1}T}]$. Here, we add noises that are uniformly from $[0, \sqrt{k^{1+\epsilon_1-\epsilon_3}T}]$ instead.


\subsection{Analysis}
Let $\zeta \in \{0, 1\}$ be the optimal action for the whole sequence, i.e. $\zeta = \arg \max_{a \in \{0,1\}}\sum_{t \leq T}\vecp^t[a]$. Let $\zeta^i \in \{0, 1\}$ be the local optimal action for the $i$-th block, i.e. $\zeta^i = \arg \max_{a \in \{0, 1\}}\vecP^i[a]$. Next, we define the \emph{local regret} as follows.

\begin{definition}Let $I \in [T]$ be an arbitrary subset of input. The \emph{local regret} $R(I)$ is
$$R(I) = \sum_{t \in I}\vecp^t[\zeta] - \sum_{t \in I}\vecp^t[a^t].$$
\end{definition}

Let us refer to the subset of blocks that uses $\proc{Algo-1}$ as $G_1$ and the
subset of blocks that uses $\proc{Algo-2}$ as $G_2$. We can see that the total regret can be expressed as
\begin{equation}
R = R(G_1) + R(G_2).
\end{equation}
Let $\tau$ be the last input such that
$$|\sum_{t \leq \tau}\vecp^t(0) -  \sum_{t \leq \tau}\vecp^t(1)| \leq 2 \sqrt{k^{1+\epsilon_1-\epsilon_3}T},$$
i.e. after time $\tau$, when a new block is processed by $\proc{Algo-2}$, the algorithm will consistently choose the expert with better accumulated payoff.
We begin with giving general bounds for $R(G_1)$ and $R(G_2)$ in terms of $\tau$ respectively.

\myparab{General bounds for $R(G_1)$ and $R(G_2)$.} Recall that the performance of using a
FPL algorithm can be described as follows.
\begin{theorem}\label{thm:fpl}Let $|x|_1$ denote $L_1$-norm. Let
\begin{itemize}
\item $D \geq |a - a'|$ for any 2 actions,
\item $R \geq |\vecp^t(a)|$ for all rewards and all actions
\item $A \geq |\vecp^t|$ for all reward.
\end{itemize}
Let $R$ be the regret from ruing a FPL over a sequence of length $T$ with noises being sampled uniformly from $[0, \frac 1 \epsilon]$. We have
\begin{equation}
\E[R] \leq \epsilon RAT + \frac D \epsilon.
\end{equation}
\end{theorem}

We first use Theorem~\ref{thm:fpl} to analyze $G_1$. Notice that for any $i$-th block in $G_1$, we have $R(\cup_{j}\vecp^j_i) \leq c_0\sqrt{k^{1+\epsilon_1}}$ for some constant $c_0$. Let $g_1$ be
the number of blocks in $G_1$. Since $b \leq \frac{T}{(1-\epsilon_0)k^{1+\epsilon_1}}$, we have
$$\E[g_1] \leq q\frac{T}{(1-\epsilon_0)k^{1+\epsilon_1}} \leq 2\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.$$
Therefore,
$$\E[R(G_1)] = \E\left[\sum_{\footnotesize{i \mbox{-th block in } G_1}}R\left(\cup_{j}\vecp^j_i\right)\right] \leq \E[g_1]c_0\sqrt k \leq 2c_0\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.$$

Next, we give a bound for $R(G_2)$. We apply Theorem~\ref{thm:fpl} again and the parameters are: $D = 2$ because we only need to choose between two actions. $R = 2(1+\epsilon_0)k^{1+\epsilon_1}$ and $A = 2(1+\epsilon_0)k^{1+\epsilon_1}$ because the size of each block is bounded by $(1+\epsilon_0)k^{1+\epsilon_1}$. Also, $\frac 1 \epsilon = \sqrt{k^{1+\epsilon_1-\epsilon_3}T}$.
A straightforward bound for the total number of input (the variable $T$ in Theorem~\ref{thm:fpl}) is $b$. But notice that after time step $\tau$, the algorithm $\proc{Algo-2}$ will
always make a \emph{correct} choice. In other words, no regret will incur after time $\tau$. Therefore, a tighter bound on the number of input is $\frac{\tau}{(1-\epsilon_0)k^{1+\epsilon_1}}$.
Thus, we have
{\small
\begin{eqnarray*}
& & \E[R(G_2)] \\
& \leq & \epsilon RAT + \frac{D}{\epsilon} \quad \quad \mbox{ \footnotesize{(The variables here are those in Theorem~\ref{thm:fpl}.)}} \\
& = & \left(\frac{1}{\sqrt{k^{1+\epsilon_1-\epsilon_3}T}}\right)\left(2(1+\epsilon_0)k^{1+\epsilon_1}\right)\left(2(1+\epsilon_0)k^{1+\epsilon_1}\right)\left(\frac{\tau}{(1-\epsilon_0)k^{1+\epsilon_1}}\right)
+ 2\sqrt{k^{1+\epsilon_1-\epsilon_3}T} \\
&\leq& c_1 \tau\sqrt{\frac{k^{1+\epsilon_1+\epsilon_3}}{T}} +2\sqrt{k^{1+\epsilon_1-\epsilon_3}T},
\end{eqnarray*}
}
where $c_1$ is a suitable constant. Summing up above, we have.
\begin{lemma}\label{lem:generalbound}Let $\tau, G_1$, and $G_2$ be defined as above. There exists two constants $c_0$ and $c_1$ such that
\begin{equation}
\E[R(G_1)]\leq 2c_0\sqrt{k^{1+\epsilon_1-\epsilon_2}T} \quad \mbox{ and } \quad \E[R(G_2)]\leq c_1 \tau\sqrt{\frac{k^{1+\epsilon_1+\epsilon_3}}{T}} +2\sqrt{k^{1+\epsilon_1-\epsilon_3}T}
\end{equation}
\end{lemma}

In the rest of our analysis, we need to consider two cases. When $\tau$ is large and when $\tau$ is small (compared to $T$).

\subsubsection{The case when $\tau$ is sufficiently small.}
Here, we consider the case where $\tau \leq k^{-\frac{\epsilon_3}2 - \frac{3\epsilon_1}{4}}T$. We have the following lemma.
\begin{lemma}\label{lem:smalltau}When $\tau \leq k^{-\frac{\epsilon_3}{2}-\frac{3\epsilon_1}{4}}T$, there exist
constants $c_0$ and $c_1$ so that our algorithm's regret $R$ satisfies
\begin{equation}
R \leq 2c_0 \sqrt{k^{1+\epsilon_1-\epsilon_2}T}+c_1\sqrt{k^{1-\epsilon_1/2}T}+2\sqrt{k^{1+\epsilon_1-\epsilon_3}T}.
\end{equation}
\end{lemma}
\begin{proof}We use Lemma~\ref{lem:generalbound}. Specifically,
\begin{eqnarray*}
R & = & R(G_1) + R(G_2) \\
& \leq & 2c_0\sqrt{k^{1+\epsilon_1-\epsilon_2}T} + c_1k^{-\frac{\epsilon_2}2-\frac{3\epsilon_1}{4}}T\sqrt{\frac{k^{1+\epsilon_1+\epsilon_3}}{T}} + 2\sqrt{k^{1+\epsilon_1-\epsilon_3}T} \quad\mbox{(Lemma~\ref{lem:generalbound})}\\
& = & 2c_0\sqrt{k^{1+\epsilon_1-\epsilon_2}T}+c_1\sqrt{k^{1-\epsilon_1/2}T}+2\sqrt{k^{1+\epsilon_1-\epsilon_3}T}.
\end{eqnarray*}
\end{proof}

\subsubsection{The case when $\tau$ is large.}
In the rest of our analysis, we focus on the case where $\tau > k^{-\frac{\epsilon_3}2 - \frac{3\epsilon_1}{4}}T$.
Let $L_i = \sum_{j \leq \ell_i}(\vecp^j_i[0] + \vecp^j_i[1])$ be the total payoffs for both actions in the $i$-th block.
We first classify each of the blocks as \emph{big blocks} and \emph{small blocks}.
\begin{definition} Let $\eta$ be a constant to be decided later.
The $i$-th block of the input is called a \emph{big block} if
$$\vecP^i[\zeta^i] \geq \frac{L_i}{2} + k^{\eta},$$
where $\frac{1+\epsilon_1}{2} < \eta < 1+\epsilon_1$ is a parameter to be determined later.
Otherwise, we call the $i$-th block a \emph{small block}. Let $\bbl \in [b]$
be the set of big blocks and $\sbl$ be the set of small blocks. Furthermore, we can
partition the set $\bbl$($\sbl$) as follows.
\begin{itemize}
\item the set $\bbl_0$ ($\sbl_0$) is the set of big groups (small groups) such that
for any $i \in \bbl_0$ ($i\in \sbl_0$), $\zeta^i = 0$.
\item the set $\bbl_1$ ($\sbl_1$) is the set of big groups (small groups) such that
for any $i \in \bbl_1$ ($i\in \sbl_1$), $\zeta^i = 1$.
\end{itemize}
Finally, we let $\bbl'$ be the set of big blocks that starts before time $\tau$,
$\bbl'_0$ be the subset of big blocks in $\bbl_0$ that starts before time $\tau$,
 $\bbl'_1$ be the subset of big blocks in $\bbl_1$ that starts before time $\tau$,
 and $\sbl'$ be the set of small blocks that starts before time $\tau$.
\end{definition}

Next, let us define the \emph{imbalance} of a block.
\begin{definition}Let $i \in [b]$ be an arbitrary block. We write $\beta(i)$ be
the \emph{imbalance} of the $i$-th block
$$\beta(i) \triangleq \frac 1 2\left|\vecP^i[0] - \vecP^i[1]\right|.$$
\end{definition}
Notice that when the $i$-th block is a big block, $\beta(i) \geq k^{\eta}$. Finally,
let $\alpha$ be the portion of blocks starting before time $\tau$ that are big. In what follows,
we shall analyze the following three cases ($\epsilon_4$ is another parameter to be decided later),
\begin{itemize}
\item \emph{Case 1.} When $\alpha$ is sufficiently large and the large blocks before time $\tau$ are
balanced, i.e.
\begin{equation}
\alpha \geq k^{-\epsilon_4} \quad \mbox{ and } \quad \frac 1 2\sum_{i \in \bbl'_1}\beta(i) \leq \sum_{i \in \bbl'_0}\beta(i) \leq 2\left(\sum_{i \in \bbl'_1}\beta(i)\right).
\end{equation}
\item \emph{Case 2.} When $\alpha$ is sufficiently large and the large blocks before time $\tau$ are imbalanced, i.e.
\begin{enumerate}
\item $\alpha \geq k^{-\epsilon_4}$ and
\item
$$\left(\sum_{i \in \bbl'_0}\beta(i) \geq 2\left(\sum_{i \in \bbl'_1}\beta(i)\right)\quad \mbox{ or } \quad \sum_{i \in \bbl'_1}\beta(i) \geq 2\left(\sum_{i \in \bbl'_0}\beta(i)\right)\right). $$
\end{enumerate}
\item \emph{Case 3.} When $\alpha$ is small, i.e. $\alpha < k^{-\epsilon_4}$.
\end{itemize}

\mypara{Case 1.} Recall that $R = R(G_1) + R(G_2)$. By Lemma~\ref{lem:generalbound}, a trivial upper bound for $R(G_2)$ is
$$R(G_2) \leq (c_1+2)\sqrt{k^{1+\epsilon_1+\epsilon_3}T}.$$
We now focus on analyzing $R(G_1)$. Wlog, let us assume that $\zeta = 0$. We may partition $G_1$ into $G_1 \cap \bbl'_1$ and
$G_1 - \bbl'_1$. Let $i$ be an arbitrary block in $G_1 \cap \bbl'_1$. Notice that
$$\vecP^i[0] \leq \frac{L_i}2 - \beta(i) \quad \mbox{ and } \vecP^i[1] \geq \frac{L_i}{2} +\beta(i).$$
When we run $\proc{Algo-1}$ on this block, our reward is at least $L_i/2+\beta(i)-c_0\sqrt{k^{1+\epsilon}}$. Therefore,
the local regret for the $i$-th block is
$$R(\cup_j\vecp^j_i) = \vecP^i[0] - \frac{L_i}{2}-\beta(i) + c_0\sqrt{k^{1+\epsilon_1}} \leq -2\beta(i) + c_0\sqrt{k^{1+\epsilon}}.$$
We now have
\begin{eqnarray*}
R(G_1) & = & R(G_1 \cap \bbl'_1) + R(G_1 - \bbl'_1) \\
&\leq & \sum_{i \in G_1 \cap \bbl'_1}\left(-2\beta(i) + c_0\sqrt{k^{1+\epsilon_1}} + \sum_{i \in G_1 - \bbl'_1}\sqrt{k^{1+\epsilon_1}}\right) \\
& = & \sum_{i \in G_1 \cap \bbl'_1}-\beta(i) + |G_1|\sqrt{k^{1+\epsilon_1}}.
\end{eqnarray*}
It is straightforward to see that
$$\E[|G_1|\sqrt{k^{1+\epsilon_1}}] = \sqrt{k^{1+\epsilon_1}}\E[|G_1|] \leq c_2 \sqrt{k^{1+\epsilon_1}} q \frac{T}{k^{1+\epsilon_1}} = c_2\sqrt{k^{1+\epsilon_1 - \epsilon_2}T}.$$
for some constant $c_2$. It remains to bound $\sum_{i \in G_1 \cap \bbl'_1}-\beta(i)$.

First, notice that the total number of blocks that start before time $\tau$ is $c_3\frac{\tau}{k^{1+\epsilon_1}}$ for some constant $c_3$.
Therefore, the total number of \emph{big} blocks is $c_3\alpha\frac{\tau}{k^{1+\epsilon_1}}$. Since within each block, its imbalance is
at least $k^{\eta}$, we have
$$\sum_{i \in \bbl'}\beta(i)\geq |\bbl'|k^{\eta} \geq\frac{c_3\tau}{k^{1+\epsilon_1}}k^{-\epsilon_4}k^{\eta}.$$
On the other hand, we have
$\sum_{i \in \bbl'}\beta(i) = \sum_{i \in \bbl'_0}\beta(i) + \sum_{i \in \bbl'_1}\beta(i)$. Together with the balanced assumption, we have
$$\sum_{i \in \bbl'_1}\beta(i) \geq \frac{c_3\tau}{3k^{1+\epsilon_1}}k^{-\epsilon_4}k^{\eta} \geq \frac{c_3(k^{-\frac{\epsilon_3}2 - \frac{3\epsilon_1}{4}})T}{3k^{1+\epsilon_1}}k^{-\epsilon_4+\eta}.$$
Finally, since the probability each block in $\bbl'_1$ belongs to $G_1$ is $q$, we have
$$\E[\sum_{i \in G_1 \cap \bbl'_1}\beta(i)] = q(\sum_{i\in \bbl'_1}\beta(i)) \geq \frac{c_3}3\sqrt{k^{-\frac{3\epsilon_1}{2}-\epsilon_2-\epsilon_3-2\epsilon_4+2\eta}T}.$$
Summing up above, the expected regret for this case is
\begin{equation}
\E[R] \leq - \frac{c_3}3\sqrt{k^{-\frac{3\epsilon_1}{2}-\epsilon_2-\epsilon_3-2\epsilon_4+2\eta}T} + (c_1+2)\sqrt{k^{1+\epsilon_1+\epsilon_3}T} + c_2\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.
\end{equation}

\mypara{Case 2.} Wlog, let us assume that
$$\sum_{i \in \bbl'_0}\beta(i) \geq 2\left(\sum_{i \in \bbl'_1}\beta(i)\right).$$
Let $\sbl'_1$ be the subset of blocks in $\sbl'$ such that for any $i \in \sbl'_1$, $\zeta^i = 1$ and
$\beta(i) \geq k^{\eta'}$, where $\eta' < \eta$ is a parameter to be determined.

Let $\gamma = |\sbl'_1|/|\sbl'\cup \bbl'|$. First we show that $\gamma = \Omega(\alpha)$. We compute the payoff of both arms up to the first block that is
after $\tau$, i.e. the blocks in $\sbl' \cup \bbl'$. First, we start with computing the payoff of the action 0 for the blocks in $\bbl'$.
\begin{eqnarray*}
\sum_{i \in \bbl'}\vecP^i[0] & = &\sum_{i \in \bbl'_0}\vecP^i[0] + \sum_{i \in \bbl'_1}\vecP^i[0] \\
& = & \sum_{i \in \bbl'_0}\left(\frac{L_i}{2} + \beta(i) \right) + \sum_{i \in \bbl'_1}\left(\frac{L_i}{2} - \beta(i) \right) \\
& = & \sum_{i \in \bbl'}\frac{L_i}2 + \sum_{i \in \bbl'_0}\beta(i) - \sum_{i \in \bbl'_1}\beta(i) \\
& \geq & \sum_{i \in \bbl'}\frac{L_i}2 + \frac 1 3 \sum_{i \in \bbl'}\beta(i) \quad \mbox{(Using the imbalance condition for $\bbl'$)} \\
& \geq & \sum_{i \in \bbl'}\frac{L_i}{2} + \frac{\alpha c_3\tau k^{\eta}}{3k^{1+\epsilon_1}}.
\end{eqnarray*}
Next, we compute the payoff of action 0 for the small blocks.
\begin{eqnarray*}
 \sum_{i \in \sbl'}\vecP^i[0]
& = & \sum_{i \in \sbl'_0}\vecP^i[0] + \sum_{i \in \sbl'_1}\vecP^i[0] \\
& \geq & \sum_{i \in \sbl'_1}\left(\frac{L_i}{2} - k^{\eta}\right) + \sum_{i \in \sbl' - \sbl'_1}\left(\frac{L_i}{2} - k^{\eta'}\right) \\
& \geq & \sum_{i \in \sbl'}\frac{L_i}2 - (\gamma k^{\eta} + (1-\gamma)k^{\eta'})|\sbl'\cup \bbl'| \\
& \geq & \sum_{i \in \sbl'}\frac{L_i}2 - \frac{c_4\tau}{k^{1+\epsilon_1}}(\gamma k^{\eta} + k^{\eta'})
\end{eqnarray*}
for some constant $c_4$.

Therefore, the total payoff of action 0 for $\sbl'\cup \bbl'$ is at least
$$\sum_{i \in \sbl' \cup \bbl'}\frac{L_i}{2}+ \frac{\alpha c_3\tau k^{\eta}}{3k^{1+\epsilon_1}}- \frac{c_4\tau}{k^{1+\epsilon_1}}(\gamma k^{\eta} + k^{\eta'}).$$

By the definition of $\tau$, the difference between two actions' payoffs for blocks in $\sbl' \cup \bbl'$ is at most $2\sqrt{k^{1+\epsilon_1-\epsilon_3}T}$. We then have
\begin{equation}\label{eq:ineqgamma}
 \frac{\alpha c_3\tau k^{\eta}}{3k^{1+\epsilon_1}}- \frac{c_4\tau}{k^{1+\epsilon_1}}(\gamma k^{\eta} + k^{\eta'}) \leq \sqrt{k^{1+\epsilon_1-\epsilon_3}T}.
\end{equation}

Suppose on the contrary that $\gamma = o(\alpha)$, then the left hand side of (\ref{eq:ineqgamma}) is $\Theta(T\cdot\mathrm{poly}(k))$ while the right
hand side is $\Theta(\sqrt T\cdot\mathrm{poly}(k))$. The left hand side would be larger than the right hand side for sufficiently large $T$. Therefore,
$\gamma \geq c_5 \alpha$ for some constant $c_5$.

Next, we consider two subcases.

\mypara{Case 2a.} $\zeta = 0$. First, it is clear that $R(G_2) \leq (c_1+2)\sqrt{k^{1+\epsilon_1+\epsilon_3}T}$. Let $i$ be an arbitrary block in
$G_1 \cap \sbl'_1$. Notice that
\begin{equation}
\vecP^i[0] \leq \frac{L_i}{2}-\beta(i) \quad \mbox{ and } \vecP^i[1] \geq \frac{L_i}{2} + \beta(i).
\end{equation}
We can see the local regret for the $i$-th block is
$$R(\cup_j \vecp^j_i) \leq -2\beta(i) + c_0\sqrt{k^{1+\epsilon_1}}.$$
We then have
$$\E[R(G_1)] = \E[R(G_1 \cap \sbl'_1)] + \E[R(G_1 - \sbl'_1)]  \leq q\left(\sum_{i \in \sbl'_1}-\beta(i)\right)+c_2\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.$$
Using the fact that $\gamma \geq c_5\alpha$, we have
$$\sum_{i \in \sbl'_1}\beta(i) \geq \frac{c_3 c_5 \tau k^{\eta'}}{k^{1+\epsilon_1+\epsilon_4}}.$$
Therefore, the total regret for this subcase is
\begin{equation}
\E[R] \leq - c_3 c_5\sqrt{k^{-\frac{3\epsilon_1}{2}-\epsilon_2-\epsilon_3-2\epsilon_4+\eta'}T} + (c_1+2)\sqrt{k^{1+\epsilon_1+\epsilon_3}T} + c_2\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.
\end{equation}

\mypara{Case 2b.} $\zeta = 1$. First, it is again clear that $R(G_2) \leq (c_1+2)\sqrt{k^{1+\epsilon_1+\epsilon_3}T}$. Let $i$ be an arbitrary block in
$G_1 \cap \bbl'_0$. Notice that
\begin{equation}
\vecP^i[0] \leq \frac{L_i}{2}-\beta(i) \quad \mbox{ and } \vecP^i[1] \geq \frac{L_i}{2} + \beta(i).
\end{equation}
We can see the local regret for the $i$-th block is
$$R(\cup_j \vecp^j_i) \leq -2\beta(i) + c_0\sqrt{k^{1+\epsilon_1}}.$$
We then have
$$\E[R(G_1)] = \E[R(G_1 \cap \bbl'_0)] + \E[R(G_1 - \bbl'_0)]  \leq q\left(\sum_{i \in \bbl'_0}-\beta(i)\right)+c_2\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.$$
Using the fact that $\sum_{i \in \bbl'_0}\beta(i) \geq 2\left(\sum_{i \in \bbl'_1}\beta(i)\right).$ we have
$$\sum_{i \in \bbl'_0}\beta(i) \geq \frac{c_3 \tau k^{\eta'}}{3k^{1+\epsilon_1+\epsilon_4}}.$$
Therefore, the total regret for this subcase is
\begin{equation}
\E[R] \leq - \frac{c_3} 3\sqrt{k^{-\frac{3\epsilon_1}{2}-\epsilon_2-\epsilon_3-2\epsilon_4+\eta}T} + (c_1+2)\sqrt{k^{1+\epsilon_1+\epsilon_3}T} + c_2\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.
\end{equation}

\mypara{Case 3.} Here, we shall use the bound developed in Lemma~\ref{lem:generalbound} for blocks in $G_1$:
$$\E[R(G_1)] \leq 2c_0\sqrt{k^{1+\epsilon_1-\epsilon_2}T}.$$
We shall focus on understanding $\E[R(G_2)]$. We need the following lemma.

\begin{lemma}\label{lem:gfpl}Let $|x|_1$ denote $L_1$-norm. Consider using a FPL over a sequence of length $T$ for two actions $\{0, 1\}$.
Let
\begin{itemize}
\item $D \geq |a - a'|$ for any 2 actions,
\item $R_t \geq |p^t[0] - p^t[1]|$ for the $t$-th input.
\item $A \geq |\vecp^t|$ for all reward.
\end{itemize}
Let $R$ be the regret from ruing the FPL with noises being sampled uniformly from $[0, \frac 1 \epsilon]$. We have
\begin{equation}
\E[R] \leq \epsilon \sum_{i \leq T}R_iA  + \frac D \epsilon.
\end{equation}
\end{lemma}

Lemma~\ref{lem:gfpl} is a generalization of the analysis for the standard FPL algorithm. The proof can be found in Appendix.
\zl{Add proof in the next iteration.}

Let $G'_2$ be the subset of blocks in $G_2$ that starts before time $\tau$. We have
\begin{equation}\label{eqn:regretg2}
R(G_2) \leq \epsilon(\sum_{i \leq G'_2}R_i)A + \frac{D}{\epsilon},
\end{equation}
where $A = 2(1+\epsilon_0)k^{1+\epsilon_1}$, $D = 2$, and $\frac{1}{\epsilon} = \sqrt{k^{1+\epsilon_1-\epsilon_3}T}$. 
Next, we assign the values of $R_i$ by using the definition of big and small blocks. Specifically, for any $i \in G'_2 \cap \sbl'$, 
we let
$R_i = 2k^{\eta}$ and for any $i \in G'_2 \cap \bbl'$, we let $R_i = 2(1+\epsilon)k^{1+\epsilon_1}$. Therefore, 
we have
$$\sum_{i \in G'_2}R_i \leq \sum_{i \in G'_2 \cap \bbl'}k^{1+\epsilon_1} + \sum_{i \in G'_2 \cap \sbl'}k^{\eta} \leq |\bbl'|k^{1+\epsilon_1}+|\sbl'|k^{\eta} \leq c_5(k^{-\epsilon_4}+k^{\eta-1-\epsilon_1})T$$
for some constant $c_5$. Now (\ref{eqn:regretg2}) becomes
\begin{eqnarray*}
R(G_2) \leq \frac{1}{\sqrt{k^{1+\epsilon_1-\epsilon_3}T}}c_6\left(k^{-\epsilon_4+k^{\eta-1-\epsilon_1}}\right)T2(1+\epsilon_0)k^{1+\epsilon_1} + 2\sqrt{k^{1+\epsilon_1-\epsilon_3}T}.
\end{eqnarray*}
Via some straightforward algebra manipulation, we can see that the total regret for this case is 
$$\E[R] = O\left(\sqrt T\left(\sqrt{k^{1+\epsilon_1-\epsilon_2}}+\sqrt{k^{-2\epsilon_4+1+\epsilon_1+\epsilon_3}}+\sqrt{k^{2\eta-1-\epsilon_1+\epsilon_3}}+\sqrt{k^{1+\epsilon_1-\epsilon_3}}\right)\right).$$

\myparab{Wrapping up the analysis.} We now set up the values of $\epsilon_1, \epsilon_2, \epsilon_3, \epsilon_4, \eta, \eta'$. To ensure the regret is $o(\sqrt{kT})$ for all cases, we need
\begin{itemize}
\item $1+\epsilon_1-\epsilon_2 < 1$ (From [$\tau$ is small], [case 1], [case 2], and [case 3])
\item $1+\epsilon_1-\epsilon_3 < 1$ (From [$\tau$ is small] and [case 3])
\item $-\frac{3}{2\epsilon_1}-\epsilon_2-\epsilon_3-2\epsilon_4+2\eta \geq 1+\epsilon_1+\epsilon_3$ (From [case 1] and [case 2b]). 
\item $\eta' < \eta$ (from [case 2])
\item $-\frac{3}{2\epsilon_1}-\epsilon_2-\epsilon_3-2\epsilon_4+2\eta' \geq 1+\epsilon_1+\epsilon_3$ (From [case 2a]). 
\item $-2\epsilon_4+1+\epsilon_1+\epsilon_3 < 1$ (From [case 3])
\item $2\eta-1\epsilon_1+\epsilon_3 < 1$ (From [case 3]).
\end{itemize}

One feasible assignment is $2\epsilon_1 = \epsilon_2 = \epsilon_3 = \epsilon_4 = \frac 1 {12}$, $\eta' = \frac 1 2 + 5 \frac 5 8 \epsilon_3$, and $\eta = \frac 1 2 + 5 \frac{11}{16} \epsilon_3$.
With this assignment, we can see that the regret is at most $O(\sqrt{k^{1-\epsilon_1/2}T})$ and the communication is $O(Tk^{-\epsilon_1})$.

\subsection{Algorithm for $n$ arms}
In this section, we generalize the algorithm for two experts (actions) to an algorithm that works for $n$ experts.
Our generalization is a recursive approach. Assume we have an algorithm $\alg$ that is able to process a system
with $n$ experts, we shall build an algorithm $\alg'$ that can process $2n$ experts as follows. We run 2 independent
copies of $\alg$ (namely $\alg_1$ and $\alg_2$) such that $\alg_1$ takes care of the first $n$ experts $a_1, a_2, ..., a_n$
and $\alg_2$ takes care of the rest of the experts $a_{n + 1}, ..., a_{2n}$. Then our algorithm $\alg'$ treat 
$\alg_1$ and $\alg_2$ as 2 experts and runs the algorithm described in the previous subsection over these two experts. 
Notice that the payoff of $\alg_1$ and $\alg_2$ are revealed at the sites. Therefore, the input structure is syntactically
matching the requirement for the 2-expert algorithm. 

We now analyze the regret for the recursive algorithm. Let the regret for $\alg_1$ be $R_1$ and the regret for
$\alg_2$ be $R_2$. We have
$$\E[\payoff(\alg_1)] \geq \max_{i \in [n]}\sum_{t \leq T}\vecp^t(i) - \E[R_1] \quad \mbox{ and } \quad \E[\payoff(\alg_2)] \geq \max_{i \in \{n + 1, ..., 2n\}}\sum_{t \leq T}\vecp^t(i) - \E[R_2].$$ 

Next, we can see that
\begin{eqnarray*}
& & \E[\payoff(\alg') \mid \payoff(\alg_1), \payoff(\alg_2)]\\
& \geq & \max\{\payoff(\alg_1), \payoff(\alg_2)\} - O(\sqrt{k^{1-\epsilon}T}) \\
& \geq & \max\{\max_{i \in [n]}\sum_{t \leq T}\vecp^t(i) - R_1, \max_{i \in \{n+1, ..., 2n\}}\sum_{t \leq T}\vecp^t(i) - R_2 \} -  O(\sqrt{k^{1-\epsilon}T}) \\
& \geq & \max\{\max_{i \in [n]}\sum_{t \leq T}\vecp^t(i) - R_1 - R_2, \max_{i \in \{n+1, ..., 2n\}}\sum_{t \leq T}\vecp^t(i) - R_1 -  R_2 \} -  O(\sqrt{k^{1-\epsilon}T}) \\
& = &  \max_{i \in [2n]} - R_1 - R_2 -  O(\sqrt{k^{1-\epsilon}T}).
\end{eqnarray*}
Therefore, 
$$\E[\payoff(\alg')] \geq  \max_{i \in [2n]} - \E[R_1] - \E[R_2] - O(\sqrt{k^{1-\epsilon}T}).$$
In other words, the expected regret of the algorithm for $n$ experts is $O(n\sqrt{k^{1\epsilon}T})$. 

\zl{Notice that here $R_1$ and $R_2$ are independent. If we can prove concentration of regret over the 2-expert algorithm, we can get a regret that is sublinear in $n$.}

Finally, let us analyze the communication cost. First, notice that the communication incurred at the end of each
block can be shared across all sites. But on the other hand, $n$ values needs to be reported from each site in the end of each block. 
Second, the communication incurred for executing $\proc{Algo-1}$ grows sublinear in $T$ and thus this kind
of cost is a smaller order cost. Therefore, the total communication cost is $O(nTk^{-\epsilon})$. This shall 
be contrasted with the trivial algorithm achieving regret $O(\sqrt{T}\log n)$ that needs $O(nT)$ communication. 
 


==> discuss.tex <==
We presented lower bounds for two natural classes of no-regret algorithms for
the distributed non-stochastic expert problem. We gave a novel algorithm
in the site-predicion model that simultaneously achieves non-trivial bounds on regret
and communication. Of course, a natural interesting open problem is to close the
gaps between the lower and upper bounds presented in the paper. 

The most interesting question is to show that \emph{any} algorithm for the
non-stochastic problem (not just of the types considered in this paper) cannot
simultaneously achieve regret asymptotically lower than $\sqrt{kT}$ and
communication asymptotically lower than $T/k$, against an \emph{oblivious}
adversary. This lower bound is true in the case of an \emph{adaptive} adversary
(see Appendix \ref{app:adaptive}. Also, finding any non-trivial algorithm
against an adaptive problem seems to be a challenging open problem.


==> jointabs.tex <==
On continuous counting and learning in a distributed system

Consider a distributed system that consists of a coordinator node connected to multiple sites. Items from a data stream arrive to the system one by one, and are arbitrarily distributed to different sites. The goal of the system is to continuously track a function of the items received so far within a prescribed relative accuracy and at the lowest possible communication cost. This class of problems is called a continual distributed stream monitoring. 

In this talk we will focus on two problems from this class. We will first discuss the count tracking problem (counter), which is an important building block for other more complex algorithms. The goal of the counter is to keep a track of the sum of all the items from the stream at all times. We show that for a class of input loads a randomized algorithm guarantees to track the count accurately with high probability and has the expected communication cost that is sublinear in both data size and the number of sites. We also establish matching lower bounds. We then illustrate how our non-monotonic counter can be applied to solve more complex problems, such as to track the second frequency moment and the Bayesian linear regression of the input stream. 

We will next consider the online non-stochastic experts problem in the continual distributed setting. Here, at each time-step, one of the sites has to pick one expert from the set of experts, and then the same site receives information about payoffs of all experts for that round. The goal of the distributed system is to minimize regret with respect to the optimal choice in hindsight, while simultaneously keeping communication to the minimum. This problem is well understood in the centralizes setting, but the communication trade-off in the distributed setting is unknown. The two extreme solutions to this problem are to communicate with everyone after each payoff, and not to communicate at all. We will discuss how to achieve the trade-off between these two approaches. We will present an algorithm that achieves a non-trivial trade-off and show the difficulties of further improving its performance. 




==> sp_ub.tex <==
Upper bound - TBD.

\begin{theorem}
There exists two constants $\epsilon_1$ and $\epsilon_2$ such that our prediction algorithm uses total communication $O(nk^{-\epsilon_1})$ and the regret is $O(\sqrt{k^{1-\epsilon_2}n})$ in white-board model.
\end{theorem}

